Bounded Quadrant System: Error-bounded Trajectory Compression on the Go

Long-term location tracking, where trajectory compression is commonly used, has gained high interest for many applications in transport, ecology, and wearable computing. However, state-of-the-art compression methods involve high space-time complexity or achieve unsatisfactory compression rate, leading to rapid exhaustion of memory, computation, storage and energy resources. We propose a novel online algorithm for error-bounded trajectory compression called the Bounded Quadrant System (BQS), which compresses trajectories with extremely small costs in space and time using convex-hulls. In this algorithm, we build a virtual coordinate system centered at a start point, and establish a rectangular bounding box as well as two bounding lines in each of its quadrants. In each quadrant, the points to be assessed are bounded by the convex-hull formed by the box and lines. Various compression error-bounds are therefore derived to quickly draw compression decisions without expensive error computations. In addition, we also propose a light version of the BQS version that achieves $\mathcal{O}(1)$ complexity in both time and space for processing each point to suit the most constrained computation environments. Furthermore, we briefly demonstrate how this algorithm can be naturally extended to the 3-D case. Using empirical GPS traces from flying foxes, cars and simulation, we demonstrate the effectiveness of our algorithm in significantly reducing the time and space complexity of trajectory compression, while greatly improving the compression rates of the state-of-the-art algorithms (up to 47%). We then show that with this algorithm, the operational time of the target resource-constrained hardware platform can be prolonged by up to 41%.

==> merge.tex <==
Compressing the raw trajectory is a fundamental part for our framework
to work appropriately in a resource-constrained environment. However,
assume that the compression rate reaches  $95\%$, a raw trajectory of $3000$
points will still leave $150$ points in the compressed
trajectory. Over time the increasing storage space needed for the
compressed trajectories is posing a challenge to the resource-constrained environment. In
this section we propose two techniques, namely trajectory merging and
trajectory ageing, to further reduce the storage space required for
the trajectories, without jeopardizing the information quality needed
for advanced tasks.


\subsection{Error-bounded Trajectory Merge}
When a new compressed trajectory segment is obtained, before
physically storing it to the storage, we apply another layer of
processing to further reduce storage. In this procedure, the incoming
segment is used as a query to search
similar historical segments in the trajectory database. If any
existing segment could represent the same path with a minor deviation,
the incoming segment is considered duplicate information and is merged
into the existing one. 

\begin{figure}[thp]
\hspace{2cm}
\includegraphics[height=4cm]{figs/merge.pdf}
\caption{Error-bounded Merge}
\label{fig:ebm}
\end{figure}

First we define the distance from a segment to a trajectory:

\begin{definition}
Given a trajectory segment $\tau=\{s, e\}$, and a trajectory
$\mathbb{T}=\{p_0,p_1,...p_n\}$, the distance from $\tau$ to
$\mathbb{T}$ is defined as the maximum value between the distance
from any point $p_i \in
\{s,e\}$ to the nearest segment $\tau^{nn} \in \mathbb{T}$, denoted
as $d^s(\tau, \tau^{nn})$, and the distance from any key point $p_j
\in \tau^{nn}$ to the segment $\overline{se}$, denoted
as $d^s( \tau^{nn}, \tau)$. Formally as
$max\{ d^s( \tau^{nn}, \tau), d^s( \tau, \tau^{nn}) \}$
\end{definition}
Note that in this definition, the distance metric we used is slightly
different from the deviation used previously. Here we use point-to-line-segment
distance instead of using point-to-line distance to reinforce the
proximity constraint between the trajectory segments. As point-to-line-segment
distance is a more strict metric, for the same
$p$ and $\overline{se}$, $d(p, \overline{se}) \leq d^s(p,
\overline{se})$, so any distance constraint under this metric will
also hold under the deviation metric.


Now we describe the merge algorithm in detail. 
Given a trajectory segment $\tau$, the algorithm for the
trajectory merge is defined in Algorithm \ref{alg:3}:

\begin{algorithm}[thp]
\caption{Error-bounded Trajectory Merge}
\textbf{Input:} Query segment $\tau=\overline{s,e}$,  merge
deviation tolerance $\epsilon^m$\\
\textbf{Algorithm:}

{\begin{algorithmic}[1]

  \STATE Create $\tau$'s expanded bounding box by expanding $\tau$'s
  bounding box by  $\epsilon^m$ in all four
  directions
  \STATE Use $\tau$'s expanded bounding box to query the historical trajectory
  database. All intersecting segments are returned and grouped by
  their trajectories as $\mathcal{G}_1=\{\tau_i,...\}, \mathcal{G}_2=\{\tau_j,...\},..., \mathcal{G}_n=\{\tau_k,...\}$
  \STATE For each segment group $\mathcal{G}_i$, find out the minimum
  segment distance from $\tau$ to any segment in the group, denoted as
  $d^{s-min}_i$
  \STATE Find the minimum $d^{s-min}_i$ for all $\mathcal{G}_i$, here we assume
  $d^{s-min}=d^{s-min}_j = d^s( \tau, \tau_k )$
  \STATE Find the update deviation bound $d^{merged}.ub$ for the nearest
  segment $\tau_k$ if we merge $\tau$ into $\tau_k$, as $d^{merged}.ub=max(
  d( s, \tau_k ), d( e, \tau_k ) ) + d_{\tau_k}$
  \IF {$d^{merged}.ub \leq \epsilon^m$}
  \STATE Associate segment $\tau_k$ to the current trajectory and vice
  versa instead of creating a new segment entity for the current
  trajectory in the
  two-way trajectory-segment index
  \ENDIF
\end{algorithmic}
}
\label{alg:3}
\end{algorithm}




Note that the expansion of the query bounding box guarantees that all
possible candidates will be included in the query results.
Figure \ref{fig:ebm} shows an example of error-bounded trajectory
merge.  The segment $\overline{p_5p_6}$ is the incoming segment and
the other three segments are from the historical trajectory database.

Now after a segment search in the spatial index, we find that
the expanded bounding box pf $\overline{p_5p_6}$ is intersecting with
the bounding boxes of $\overline{p_1p_2}$ and $\overline{p_2p_3}$,
both of which belong to the same
trajectory. In this case, the minimum segment-to-trajectory distance from
$\overline{p_5p_6}$ is equal to the segment-to-segment distance from
$\overline{p_2p_3}$ to $\overline{p_5p_6}$, which is equal to $d(p_2,p_5)$. Assume
that  $d(p_2,p_5) + d(\overline{p_2p_3}) \leq \epsilon^m$, meaning
the deviation bound after merge is less than or equal to the merge threshold
$\epsilon^m$, we could merge $\overline{p_5p_6}$ into
$\overline{p_2p_3}$. And $\overline{p_2p_3}$ has an updated deviation
bound of $d(p_2,p_5) + d(\overline{p_2p_3}) $ and is now also linked to
the current trajectory in addition to its original trajectory. 
$\overline{p_5p_6}$ is safely discarded.

\subsection{Trajectory Ageing}
Despite the space saved from merging similar trajectories, another
scheme called ageing is used to further improve the utilization of storage
space. The intuition is that newer and older trajectories should not
bear the same significance in the historical trajectory database,
because  more recent trips represent the moving object's recent travel
patterns better and should be regarded of greater interest in our framework.
And the procedure is to re-run compression algorithms on the existing
trajectories that are already compressed, but with a greater deviation
tolerance, so that the compression rate will be further improved.

Consequently, we propose an ageing strategy for the historical
trajectories stored. We use a logistic function to describe the
decay of trajectory significance over time:
\begin{equation}
s=\frac{1}{1+e^{\alpha\times i-\overline{m}}}
\end{equation}

$\overline{m}$ is the maximum time unit we keep a trajectory in the
historical trajectory database. In this case we set the time unit to
be week and the maximum time a trajectory is kept is 10. The
decay function, depicted in Figure \ref{fig:dec}, gives a smooth
decaying significance curve, which is defined by setting $\alpha=1.5$ and
$\overline{m}=10$. 

\begin{figure}[tph]
\hspace{1.5cm}
\includegraphics[height=4cm]{figs/decay.pdf}
\caption{Significance Decay}
\label{fig:dec}
\end{figure}

With the decaying significance, we could apply greater deviation
tolerance and hence achieve further compression for the historical trajectories
that have greater ages. The older the data is, the less significant
the data is to the framework, therefore
the greater the deviation tolerance should be. This means the
trajectories should be recompressed to a more coarse form. In this
step, we use Algorithm \ref{alg:2} again on the compressed trajectories, and
the new deviation threshold is defined as:
\begin{equation}
\epsilon^a = \frac{\epsilon^d}{s} = \epsilon^d \times (1+e^{\alpha\times i-\overline{m}}) 
\end{equation}

Assume that $\mathbb{T}'$ is the new trajectory after applying the
ageing process on trajectory $\mathbb{T}$, the deviation of
$\mathbb{T} '$ should satisfy:
\begin{equation}
d(\mathbb{T} ') +\epsilon^d \leq \epsilon^a 
\end{equation}

Under such setting,  we guaratee $\mathbb{T} '$ is still
error-bounded. The bounding boxes for the segments in $\mathbb{T} '$
are adjusted according to the new deviation bound $d(\mathbb{T} ') +\epsilon^d$.

==> storage.tex <==
\begin{figure}[htp]
\hspace{0.1cm}
\includegraphics[height=7cm]{figs/index.pdf}
\caption{Storage and Index}
\caption*{The sub-diagram ``Spatial Index'' visualises the compressed
  trajectories in the R-Tree~\cite{Guttman:1984:RDI:602259.602266} spatial index. The sub-diagrams ``Segment
  Index'' and
  ``Waypoint Index'' describe the storage structure of the information
that is linked to the index trajectories and segments.}
\label{fig:idx}
\end{figure}

In our framework, the efficient organization of data is essential to
almost every task. To be specific, we need to store the compressed 
trajectories in a well-designed index structure as a historical database,
which is used to speed up trajectory
matching for either trajectory merging, ageing, waypoint mining or
other advanced tasks in future. 

Here we propose to use a multi-layer index structure to manage the
data, as shown in Figure \ref{fig:idx}. The key
components and mechanisms are as follows:
\begin{itemize}
\item A spatial index (R-Tree \cite{Guttman:1984:RDI:602259.602266} as an example) to enable efficient query and access to
  trajectory segment.
\item A two-way reverted list as the segment index that maintains the
  relations between trajectories and their segments.
\item A waypoint index that index rectangles which represent waypoint
  areas in the spatial domain.
\end{itemize}

The three indices are designed to work together as a database for the
historical data from the same individual. The Spatial index links 
trajectory segments with bounding
boxes, for fast intersection queries during trajectory segment
matching and waypoint area mining. Given a query trajectory segment,
represented as a bounding box, the index will return the intersecting
bounding boxes in $\mathcal{O}(\log_Mn)$ time complexity, where $M$ is the
maximum number of entries in a R-Tree page and $n$ is the number of total
points.

The two-way inverted list maintains the trajectory structure by
keeping records of the relation between segments and trajectories. It
is able to return the information on which segments belong to a trajectory, as
well as a trajectory contains which segments. For a query from either
side to the other, the time complexity is generally $\mathcal{O}(\log n)$, where
$n$ is the number of trajectories or segments.

The waypoint index is a simple list of waypoint areas, represented by
the rectangles in the spatial index.

In the following sections we address the sub-problems described previously
in the Overview section.


==> waypoint.tex <==


\begin{algorithm}[thp]
\caption{The Waypoint Search Algorithm}
\textbf{Input:} Historical trajectories $\{\mathbb{T}_i\}$, the newly
added trajectory $\mathbb{T}$, existing waypoints $\{wp_i\}$ in the
waypoint index, waypoint size $r$, minimum intersecting trajectories $n^{traj}_{min}$ \\
\textbf{Output:} An updated waypoint index $\{wp_i\}$\\
\textbf{Algorithm:}

{\begin{algorithmic}[1]
  \FOR{ Each segment $\tau_i \in \mathbb{T}$}
  \STATE Use $\tau_i$'s bounding box as a query to search for intersecting
  segments $\{\tau_j\}$ in the trajectory index
  \STATE If the number of intersecting trajectories is smaller than
  $n^{traj}_{min}$, skip current segment and continue the loop
  \STATE Calculate the density score $s^{dnst}$ and the dispersion score $s^{disp}$ for $\tau_i$ 
  \STATE Calculate $s^{wp}$ using Equation \ref{eqn:wps}
  \STATE Compare $s^{wp}$ against the lowest score for the existing
  waypoints, denoted as $s^{wp_i}_{min}$
  \IF { $s^{wp} < s^{wp_i}_{min}$}
  \STATE Return
  \ELSE
  \STATE Compare $\tau_i$'s bounding box against those of the existing
  waypoints
  \STATE If $\tau_i$ is too close to an existing waypoint area $wp_j$,
  compare their waypoint scores and keep only the one with a higher
  score
  \STATE Replace the existing waypoint with the lowest score 
  \ENDIF
  \ENDFOR
\end{algorithmic}
}
\label{alg:wps}
\end{algorithm}


In long-term tracking applications, discovering the significant
waypoint areas for an individual is another crucial task that can benefit
many advanced tasks greatly. A waypoint area is a location at where many
trajectories join paths but part ways afterwards. By
finding these areas, we are able to assist many advanced applications
on the framework such as trip prediction.

We introduce a metric called the waypoint score to measure the significant areas in a moving
object's travel history. It consists of two aspects: \textit{density}
and \textit{dispersion}. \textit{Density} describes the concentration
of trajectories passing through the area, while \textit{dispersion}
summarizes how diverse the directions are for these
trajectories. As in our framework, a trajectory segment is also considered
conceptually representing an area, we use the length of segments to
normalize the waypoint scores so that places where 
momentous turns happen repeatedly will be captured. Formally, we have:
\begin{definition}[Waypoint Score]
For a given segment $\tau$, the waypoint score $s^{wp}$ of $\tau$'s
center is defined as:
\begin{eqnarray}
s^{wp}_\tau = \frac{|\{\mathbb{T}_i'\}|\times std( \{\theta_{\tau_j}\}))^\gamma}{length(\tau)}
\label{eqn:wps}
\end{eqnarray}
\label{def:wps}
\end{definition}
where $\frac{|\{\mathbb{T}_i'\}|}{langth(\tau)}$ is the number of trajectories passing
through the area divided by the length of the segment, $\{\theta_{\tau_j}\}$ is the set of heading
angles for all the trajectories segments passing the area, and $\gamma$
is a parameter to adjust the relative weights between the two
aspects. The $length(\tau)$ component normalizes the score by
the length of the trajectory, so that denser areas are favored.

The waypoint score measures the two aforementioned aspects of a waypoint area
in a mathematical way, while providing means for a balance between the two.
To fit the scenario of the framework, we perform the
search procedure is performed whenever a new trajectory's 
addition is completed. To search for waypoints from the historical trajectories, we devise
the waypoint discovery algorithm in Algorithm \ref{alg:wps}. In this
efficient search algorithm the segments are used as waypoint
candidates, with the waypoints considered to be centered at the center the segments.







